Dependent Type Systems as Macros

We present Turnstile+, a high-level, macros-based metaDSL for building dependently typed languages. With it, programmers may rapidly prototype and iterate on the design of new dependently typed features and extensions. Or they may create entirely new DSLs whose dependent type "power" is tailored to a specific domain. Our framework's support of language-oriented programming also makes it suitable for experimenting with systems of interacting components, e.g., a proof assistant and its companion DSLs. This paper explains the implementation details of Turnstile+, as well as how it may be used to create a wide-variety of dependently typed languages, from a lightweight one with indexed types, to a full spectrum proof assistant, complete with a tactic system and extensions for features like sized types and SMT interaction.

==> app-macro.tex <==
\section{Style and Glossary}\label{app:style}

This section summarizes the various style choices used in the paper, and also
presents some macro terminology that may help with reading the paper.

\subsection{Macros Glossary}

\begin{itemize}

\item A \emph{syntax object} is the Racket AST representation. It's a tree of
  symbols, infused with context information such as source locations, the
  program's binding structure, and even arbitrary user-specified
  metadata. Syntax objects originated in Scheme~\cite{dybvig1992} and represent
  a compromise between the purely symbolic ``code-as-data'' Lisp s-expressions,
  which lose all context information, and traditional AST structures, which are
  not composable (\ie, cannot write macros that generate or use other macros).

\item \emph{Syntax patterns} deconstruct syntax objects, binding \emph{pattern variables} to different parts of a syntax object, which are themselves syntax objects.

\item \emph{Syntax templates} construct syntax objects. They may reference
  pattern variables, whose corresponding syntax object gets embedded into the
  constructed syntax object. They are typically used in conjunction with a
  quasiquoting system and thus syntax templates may be interleaved with host
  language code that constructs some pieces of the syntax object.

\item \emph{Syntax properties} are key-value pairs associated with syntax object
  nodes. We use syntax properties to propagate type and other meta information
  about a piece of syntax.

\end{itemize}

\subsection{Style}

In the paper, to help readability, we often stylize code with colors or abbreviations. This section summarizes a few of our choices.

\begin{itemize}

\item Square brackets have the same semantics as round parentheses. They are
  typically used, according to various conventions, to help readability.
\item \pat{syntax pattern} positions, which deconstruct syntax objects, are
  highlighted with gray. Like most typical pattern matchers, each separate
  language construct itself determines which positions are syntax pattern
  positions. For example, a macro definition's input is frequently a pattern
  position, as is the first position after a \ttt{\stxwith} directive in a
  macro definition.
\item \stx{syntax template} positions, which construct syntax objects, are in
  blue. A programmer typically constructs a syntax object with syntax
  constructor expression, \ie, the symbols \ttt{\#'} followed immediately by
  the template. This expression is commonly used as a macro definition's
  output, for example. Some language constructs, however, have positions that
  are implicitly syntax templates; an example is a \Turntwo \ttt{\deftyrule}.

When there are nested positions, e.g., for a macro defining macro, we might
instead enclose the syntax template with \ulltt\ulrtt, so that the coloring of
any nested pattern and syntax template positions are not obscured.

\item The name being defined (e.g., a macro, typerule, function, etc.) is always in \textbf{bold}.
\item Pattern variables representing expanded syntax objects, or constructs in
  a target language, \eg, \texttt{\er{\lm}}, are marked with an overline.
\item \emph{Syntax classes}, which additionally constrain the shape of pattern
  variables in a syntax pattern, are written with a superscript.

\end{itemize}




\section{Macro System Features}\label{app:macrofeatures}

This section, beginning with table~\ref{tab:macrofeatures}, summarizes the
macro system features used in the paper, and their availability in other
languages. While, to our knowledge, Racket is the only language that currently
combines all the features needed for ``dependent type systems as macros'',
Racket's macro system continues to influence even non-Lisp modern
languages~\cite{disney:thesis, ocaml:phases, burmako:scala, rust:scopes,
  haskellwrong}, so many of the needed features are gradually being adopted into
other systems.


\begin{table}[htbp]

\begin{tabular}{lllllllll}
                            & Racket & Lisp & Clojure & Scala & Rust & Julia & Elixir & Crystal \\
\hline
Procedural macros           & X      & X           & X       & X     &      & X     & X      &         \\
Quasiquotation              & X      & X           & X       & X     & X    & X     & X      & X       \\
Syntax pattern matching     & X      &             &         & X     & X    &       &        &         \\
Extensible pattern matching & X      &             &         & X\textsubscript{1}   &      &       &        &         \\
Automatic hygiene           & X      &             &         &       & X    & X     & X      &         \\
Syntax properties           & X      & X\textsubscript{2}         & X\textsubscript{3}     & X\textsubscript{4}   &      &       &        &         \\
Macro-defining macros       & X      & X           & X       &       &      &       &        & X       \\
Identifier macros           & X      & X           & $\sim$\textsubscript{5}&       &      &       &        &         \\
Local expansion             & X      & X           & $\sim$\textsubscript{5}&       &      &       &        &         \\
Interposition points        & X      &             &         &       &      &       &        &
\end{tabular}

\begin{enumerate}
    \item Referred to as ``extractor macros''
    \item Referred to as ``property lists''
    \item Referred to as ``metadata''
    \item Referred to as ``attachments''
    \item Clojure does not have symbol macros or expansion in the environment of local macro definitions, but they can be added as a library. See \url{https://github.com/clojure/tools.macro}.
\end{enumerate}
\caption{Macro system features used in the paper, and their availability in other macro systems.}
\label{tab:macrofeatures}
\end{table}

\subsection{Procedural macros}

Procedural macros are syntax transformations defined in a general-purpose language supporting arbitrary computations. They are essential to allow arbitrary type-checking logic during expansion.

\subsection{Quasiquotation and syntax pattern matching}

With quasiquotation, macros construct their expansion using syntax matching the textual form of the language, plus escapes for inserting computed elements.
%
Similarly, macros using syntax pattern matching deconstruct the AST of macro invocations using syntax matching the textual form of the language.
%
We use pattern matching and quasiquotation to give type rule macros relatively readable syntax, even without the \Turntwo DSL layer.

\subsection{Extensible pattern matching}

\Turntwo types expand into a common internal representation which enables simple implementations of type equality and substitution. Pattern matching this internal representation is verbose. we use Racket's \emph{pattern expanders}, e.g., in section~\ref{subsec:patexpanders}, to abstract away the internal representation and create simple pattern forms for each type constructor.

\subsection{Automatic hygiene}

Program transformations that introduce temporary variables or references to procedure bindings that may be shadowed need to take care to avoid name capture. Manual solutions include using an operation to generate unique names, and namespace-qualifying references. Macro systems supporting automatic hygiene~\cite{dybvig1992} avoid capture without any such manual intervention. Automatic hygiene is useful for types as macros because it keeps type rules concise. Racket uses the set of scopes hygiene algorithm, which works well with local expansion \cite{setsofscopes}.

\subsection{Syntax properties}

Syntax properties are key-value pairs that may be attached to syntax during expansion, and communicate extra information about syntax between macros.
%
We annotate typechecked forms with a syntax property in order to communicate the inferred type to the parent form's expansion.

\subsection{Macro-defining macros and identifier macros}

In a system supporting macro-defining macros, the expansion of one macro may define another. Identifier macros, also known as symbol macros, allow an identifier to be bound to a macro that expands when the identifier is used in reference position.
%
We use macro-defined identifier macros to cause references to typed variables to be annotated with their type.
%
The \Turntwo DSL is also an example of a macro-defining macro, as are uses of the \ttt{\deftyrule} macro to define type rule macros.

\subsection{Local expansion}

Macro systems with local expansion allow macros to request the expansion of subexpressions, including in the environment of local variable and macro bindings. We use local expansion to typecheck subexpressions and access their inferred type while typechecking the parent expression. Racket's approach to local expansion is discussed in \citet{fcdf:macrosworktogether}.

\subsection{Interposition points}

Racket's expander automatically inserts hooks at various points, e.g., the
\ttt{\#\%app} macro at each function application and the \ttt{\#\%datum}
macro at each literal datum (like a number), to allow customizing the behavior
of these and other constructs such as modules and the REPL.  By redefining
these macros, types as macros can add typechecking to the expansion of these
syntactic elements.

\subsection{Dynamic Extent Parameters}

\Turntwo itself further inserts overloadable hooks for even more
extensibility. This allows, for example, changing the type checking relation
without rewriting all the rules. These hook points are denoted with a box, \eg,
\param{norm}. They are implemented with \emph{parameters}, a more-controlled
form of dynamic binding~\cite{fluidthreads}.

%% \subsection{Interleaving Semantics}
%% \begin{figure}
%%   \includegraphics{diagram.pdf}
%%   \caption{Example of the interleaving}
%%   \label{fig:diagram}
%% \end{figure}

%% Combined, the above features allow us to interleave macro expansion, type
%% checking, and evaluation, and to communicate information across each stage
%% effectively.
%% In \fullref[left]{fig:diagram}, we give an example of a term as it proceeds through
%% the interleaved macro expansion and type checking process, while in \fullref[right]{fig:diagram}, we show an example of the interleaving of macro expansion, type
%% checking, and evaluation.
%% Specifically, we show the expansion of an equality type \ttt{(= 2 (+ 1 1))}.
%% Without type level reduction, this elaborates each subexpression into the
%% type-annotated version (denoted by the \(\tau\) subscript), before generating
%% the fully elaborated run-time representations (denoted by the \ttt{R} subscript).
%% The type-annotated versions represent the output of type-rule macros, while the
%% run-time representations represent the output of the reduction-rule macros.
%% Without dependent types, the type-annotated and run-time representations are the
%% same.
%% However, once we support dependent types and reduction rules as macros, they are
%% different and require the reflection process described in \fullref[]{sec:dep}.

%% Notice that, on the right of the figure with reduction during type-checking, we
%% end up with a run-time subterm that must be interleaved with type-annotated terms.
%% Supporting this, particularly when any term (such as a function defined in
%% another module) can be evaluated at expansion time, is the key challenge in the
%% type systems as macros approach, which we solve using many of the above macro
%% system features.


%\subsection{syntax pattern matching}

%We make heavy use of pattern-match-based macros, as pioneered by ~\citet{macro-by-example}, and enhanced by~\citet{culpepper:syntaxparse}.
%In particular, we use \stxparse and its pattern combinators.

%Macro-based macros are a very old feature and are undoubtedly available in many modern macro systems, e.g., Rust.\footnote{\url{https://doc.rust-lang.org/reference/macros-by-example.html}}

%\subsection{syntax quasiquoting}

%This feature is standard in most metaprogramming systems these days.

%\subsection{\texttt{local-expand}}

%This is the ability to expand an arbitrary piece of syntax and is also widely available.

%\subsection{syntax properties}

%Syntax properties associate arbitrary key-value pairs with an AST node. Many
%other languages have reflection capabilities that allow this.

%\subsection{overloadable core-forms}

%We rely on Racket's overloadable core forms, e.g., \appm, \lmtt, and \datum, to inject type rules.

%\subsection{procedural macros}

%\subsection{identifier macros}

%\subsection{non-expression macros}
%e.g., pattern expanders


%\subsection{hygiene}

%e.g., \cite{setsofscopes}



==> sandbox.tex <==
% intro

% macros as libraries

With conventional language, experimenting with a language means extending the
compiler. With macros, experimental features may be distributed as a library,
and thus only interested users need to deal with it.
Examples
- ornaments?
- pattern synonyms
- size types

% pattern synonyms

Macros allow experimenting with language features that do not typically allow abstracting, \eg pattern matching, as a modular library. Typically, abstractions over these parts of the language require extending the compiler~\cite{pattern synonyms Haskell 16 Pickering et al, McBride 2009 Strathclye Haskell Extension, Adga}
- also, abstracting over datadefinitions

% sec 2: racket and turnstile primer
(Note that the name of the macro, which we \defname{bold} in this paper, is
always \emph{included} as the first part of a macro's input pattern shape.)


% sec 1
the interleaving of checking and transformation inherent in our macro-based
approach will be key for implementing dependent types, where evaluation (ie normalization, a form
of transformation) is interleaved with checking

% sec1 stx obj
Syntax objects the raw symbols of an s-expression, infused with context
information like binding and source location. It represents a compromise
between the purely homoiconic lisp s-expression symbols and a transitional
language that is parsed into an s-exression. The former needlessly throws away
context information from a program, a huge sacrifice just to claim ``code is
data'', while the latter requires a complicated parse step that severely
constraints any macro system so that abstractions are not composable \eg, you
cannot write a macro that generates another macro. In contrast, a syntax object
still mirrors the concrete syntax exactly, so parsing is trivial, and is thus
composable, but does not lose critical context info. The tradeoff is that stx
objs cannot be manipulated with plain list functions, like in lisp; instead
they require their own ``lifted'' api.

% sec 2 primer
- show flip rule where check is implemented with check
- mention that turnstile defaults to this if check rule not given

% sec 2 primer
- add ``ann'' rule

% section 3
% Type : Type
For now, we assume that Type : Type. That is, Type is a special macro that expands to a syntax object with itself as its type.





% extensional subst/transport identity eliminator
- mention that we do this on purpose, and reference later when talking about managing extensions

% pattern matching
- pat-complete?
- pat->ctxt
- mention that we only use simple pattern matching where we must have all combination of cases, but we are working on a case splitting algorithm

- mention that we use ``first match'' semantics for pattern matching?
  - where does this differ from ``case split'' semantics?

